Demand-Adaptive Route Planning and Scheduling for Urban Hub-based High-Capacity Mobility-on-Demand Services

In this study, we propose a three-stage framework for the planning and scheduling of high-capacity mobility-on-demand services (e.g., micro transit and flexible transit) at urban activity hubs. The proposed framework consists of (1) the route generation step to and from the activity hub with connectivity to existing transit systems, and (2) the robust route scheduling step which determines the vehicle assignment and route headway under demand uncertainty. Efficient exact and heuristic algorithms are developed for identifying the minimum number of routes that maximize passenger coverage, and a matching scheme is proposed to combine routes to and from the hub into roundtrips optimally. With the generated routes, the robust route scheduling problem is formulated as a two-stage robust optimization problem. Model reformulations are introduced to solve the robust optimization problem into the global optimum. In this regard, the proposed framework presents both algorithmic and analytic solutions for developing the hub-based transit services in response to the varying passenger demand over a short-time period. To validate the effectiveness of the proposed framework, comprehensive numerical experiments are conducted for planning the HHMoD services at the JFK airport in New York City (NYC). The results show the superior performance of the proposed route generation algorithm to maximize the citywide coverage more efficiently. The results also demonstrate the cost-effectiveness of the robust route schedules under normal demand conditions and against worst-case-oriented realizations of passenger demand.

==> fleet_robust.tex <==
\section{Fleet management with candidate routes}

We summarize the list of variables used in this section in Table~\ref{notation}. 
\begin{table}[htbp!]
	\setstretch{1.2}
	\centering
	\caption{Table of notation}
	\label{notation}
	\begin{tabular}{p{3cm}p{10cm}}
		\hline
		Notation & Description \\ \hline
		&\textbf{Variables}\\ \hline
		$X_{i}$ & Expected passenger demand in zone $i$.\\
	    $x_{s,i}^{max}$ & Actual passenger demand aboard at zone $i$ for route $s$. \\
	    $x_{s,i}^{min}$ & Actual alighting passenger demand at zone $i$ for route $s$.\\
	    $t_{s,i}$ & Planned dwelling time for route $s$ at zone $i$.\\
	    $T^{travel}_s$ & Total driving time of route $s$.\\
	    $T^{boarding}_s$ & Total amount of boarding and alighting time of route $s$.\\
	    $h_s$ & Headway of route $s$.\\
	    $y_s$ & Number of vehicles assigned to route $s$. \\
	    $B$ & Total number of available vehicles for a given planning period. \\
	    $Q_{s,i}$ & Induced passenger demand for the DAT service at zone $i$ for route $s$.\\
	    $\tilde{Q}_{i}$ & Passenger demand who choose to user alternate travel mode. \\
	    $\delta_{s,i}$ & Indicator variable. $\delta_{s,i}=1$ if route $s$ serves zone $i$, and 0 otherwise.\\
	    $c_r$ & Single trip price paid by the passenger. \\
        \hline
	\end{tabular}
\end{table}

The fleet management of interest here is to determine the allocation of a fleet of $B$ vehicles to the set of candidate routes $\mathcal{R}$ and the corresponding frequency of each route, termed by the headway frequency $h_s$. We follow the framework in~\cite{gkiotsalitis2017exact} to develop the mathematical formulation for the DAT frequency problem with given candidate routes. The objective of the fleet management is to identify the optimal assignment between vehicle resources and candidate routes and the corresponding route frequency, where passengers may make their choices accordingly to select their travel mode, so that the total operation revenue is maximized. As for the operation revenue, we explicitly consider three contributing components: (1) the operation costs, (2) the gain in externalities and (3) the out-of-pocket cost paid by the passengers, where each components can be mathematically expressed as:
% \begin{subequations}
% \begin{align}
% F_{operation}&=c_o \sum_{s\in\mathcal{R}} (T^{travel}_s+T^{boarding}_s)y_s\\
% F_{revenue}&=c_r\sum_{s\in\mathcal{R}} \sum_{i\in V} Q_{s,i}\delta_{s,i}\\
% F_{saving}&=\sum_{s\in\mathcal{R}} \sum_{i\in V} e_{i}Q_{s,i}\delta_{s,i}
% \end{align}
% \end{subequations}
% where $c_o$ denotes the operation cost per unit operation time, $c_r$ is the flat rate ticket price per passenger and $e_{i}$ is the corresponding savings in externality per served passenger. We can formally write the nominal fleet management problem in our study as:
% \begin{equation}
%   \min_{y,h,t,X}\quad \omega_oF_{operation}-\omega_sF_{saving}-\omega_rF_{revenue} \label{eq:obj}
% \end{equation}
% subject to
% \begin{subequations}
% \begin{align}[left ={\mathcal{H}(X)  \empheqlbrace}]
%     &t_{s,i} \geq t_b X_ih_{s,i} \label{eq:dwell_time}\\
%     &T_{s}=T^{travel}_s+\sum_i t_{s,i}\delta_{s,i} \label{eq:route_time}\\
%     &y_sh_s\geq T_s^{trip}\kappa_s+\sum_i \delta_{s,i}t_{s,i} \label{eq:service_frequency}\\
%     &\sum_{s\in\mathcal{R}} y_s\leq B \label{eq:fleet_size} \\
%     &y_s\leq B\kappa_s, t_{s,i}\leq M \kappa_s, \kappa_s\in\{0,1\},y_s\in \mathbbm{I}
% \end{align}
% \end{subequations}
% \begin{subequations}
% \begin{align}
%     &T_{s,i}=\frac{h_s}{2}+T^{travel}_{s,i}+\sum_{j\in Prec(s,i)}t_{s,j}\delta_{s,j} \label{eq:passenger waiting}\\
%     &U_i(t,h)=\frac {e^{{c_1^{DAT} T_{s,i}+c_2^{DAT}c_r+b^{DAT}}}}{\sum_{m\in\mathcal{M}}e^{{c_1^MT^M_i+c_2^Mc^M_i+b^M}}} \label{eq:demand_split}\\
%     &X_i\leq \sum_s\dot{X}_iU_i(t,h)\\
%     &X_i\leq \sum_s\dot{X}_i\kappa_s\delta_{s,i}\\
%     & X_i\geq 0 \label{eq:integer_cons}
%     \end{align}
% \end{subequations}


\begin{subequations}
\begin{align}
F_{operation}&=c_o \sum_{s\in\mathcal{R}} (T^{travel}_s+T^{boarding}_s)y_s\\
F_{revenue}&=c_r\sum_{s\in\mathcal{R}} \sum_{i\in V} Q_{s,i}\delta_{s,i}\\
F_{saving}&=\sum_{s\in\mathcal{R}} \sum_{i\in V} e_{i}Q_{s,i}\delta_{s,i}
\end{align}
\end{subequations}
where $c_o$ denotes the operation cost per unit operation time, $c_r$ is the flat rate ticket price per passenger and $e_{i}$ is the corresponding savings in externality per served passenger. We can formally write the nominal fleet management problem in our study as:
\begin{equation}
  \min_{y,s,X,L}\quad \omega_oF_{operation}+\omega_wF_{waiting}+\omega_l \sum_i L_{i}\label{eq:obj}
\end{equation}
subject to
\begin{subequations}
\begin{align}[left ={\mathcal{H}(X)=  \empheqlbrace}]
    &y_sh_s\geq T_s \label{eq:service_frequency}\\
    &h_s\geq h^{min} \label{eq:min_freq}\\
    &\sum_{s\in\mathcal{R}} y_s\leq B \label{eq:fleet_size}
\end{align}
\end{subequations}
\begin{subequations}
\begin{align}
    &\sum_s\sum_{i\in R_s^F} h_sX_{s,i}\delta_{s,i}\leq C \label{eq:to_hub_capacity}\\
    &\sum_s\sum_{i\in R_s^T} h_sX_{s,i}\delta_{s,i}\leq C \label{eq:from_hub_capacity}\\
    &\sum_s X_{s,i}+L_{i}= \bar{D}_i\\
    & X_i\geq 0 \label{eq:integer_cons}
    \end{align}
\end{subequations}


where the set $\mathcal{H}(X)$ describes the constraints for the frequency planing of candidate routes as a function of the passenger demand, and equations~\ref{eq:passenger waiting} measures the expected waiting and traveling time of route $s$ for passengers at station $s$ and~\ref{eq:demand_split} denotes the rational choices made by passengers depending on the cost and travel time and the planned DAT services. Specifically, equation~\ref{eq:dwell_time} gives the dwelling time at each station $i$ of route $s$, where we use $t_b$ to represent the boarding and alighting time per passenger and the dwelling time therefore depends on the maximum between the boarding and alighting time. Equation~\ref{eq:route_time} calculates the total trip time as the sum of travel time between stations and the dwelling time at each station. And equation~\ref{eq:service_frequency} restricts the headway between successive vehicles based on the number of assigned vehicles and the route trip time. Finally, equation~\ref{eq:fleet_size} states that the total assigned vehicles shall not exceed the available number of vehicles for the current planning time period. 

Given the set of candidate routes, the optimization problem aims at identifying the optimal service headway $h_s$ and assigned vehicles $y_s$ for each route $s\in\mathcal{R}$ based on the responses from the passengers. Note that the nominal fleet management problem described by equations~\ref{eq:obj}-~\ref{eq:integer_cons} considers known passenger demand as a point estimation (such as expected value). Nevertheless, for the proactive planning of DAT service within a short time interval, the passenger demand may vary significantly and the planned service based on expected passenger demand is unlikely to align with the actual realization of demand profile. This may lead to the situation where there is overly supply in certain routes due to the revealed demand being significantly lower, while there are insufficient vehicles to serve the actual demand on other routes.     The objective of the fleet optimization is to maximize the energy savings and service revenue while minimizing operation and capital cost (all converted to equivalent monetary cost), under the worst possible passenger realization.

We note that the nominal problem as described by equations~\ref{eq:obj}-~\ref{eq:integer_cons} is a nonlinear and nonconvex integer programming problem, which is difficult to solve directly due to the existence of bilinear constraints and the nonlinear relationship between passengers's response and the planned headway and fleet configuration. 
% \begin{equation}
%   \begin{aligned}
% \text{maximize}\; & F_{energy}+F_{revenue}-F_{operation}-F_{capital}\\ 
% & F_{energy}=\sum_{i\in V}\sum_{k\in\mathcal{R}} e_{i} q^k_{i}\\
% \end{aligned}  
% \end{equation}
In this regard, if the interval of demand is supplied, we are dealing with a two-stage robust scheduling of fleet headway given the set of candidate routes. We consider the realistic scenario where passengers have access to both planned HHMoD service and other trip modes and they will greedily choose the trip service with the highest utility (travel time and trip cost). The travel time of a passenger at location $i$ using route $k$ consists of the transit operation time between each pair of stations, the expected waiting time at the location and the cumulative loading (unloading) time before arriving at her final destination. In the first stage, the main problem becomes that the decision maker determines the set of routes to operate and the corresponding headway $x_k$. Then for the second stage, we have the recourse problem where passengers will react to the planned headway with the worst realization of possible spatial distribution and the selection of alternate travel mode. In summary, the objective function of the fleet optimization becomes:
\begin{equation}
  \begin{aligned}
\min_{y,h}\; & \omega_oF_{operation}+\max_{p\in\mathcal{P}}\min_{X\in \mathcal{F}(y,h,p)}\omega_wF_{waiting}+\omega_l \sum_i L_i\\ 
\end{aligned}  
\label{eq:robust}
\end{equation}
where we define the uncertain set $\mathcal{P}$ as:
\begin{equation}
    \mathcal{P}=\{p|p_i\in\mathbbm{1}, \sum_i p_i=\Tau\}
\end{equation}
and the set $X\in\mathcal{F}(y,h,p)$ can be represented by equation~\ref{eq:demand_split} and the following equality constraint
\begin{subequations}
\begin{align}
    \sum_s X_{s,i}+L_i=\bar{D}_i+p_iZ_i, \forall\,i\in V
\end{align}
\end{subequations}
$\mathcal{F}$ and $\mathcal{P}$ constitute the uncertainty set of travel demand and the level of budget available for the DAT planner to address the uncertainties. The recourse problem in Problem~\ref{eq:robust} can be converted into a single maximization problem by utilizing its dual representation. This allows us to solve the robust fleet optimization problem following the column-and-constraint generation algorithm as in~\cite{zeng2013solving}. 

For the recourse problem, we can easily write it as:
\begin{eqnarray}
\begin{aligned}
    \max_{p} \min_{X}\quad & \sum_{s\in\mathcal{R}}\sum_{i\in V} \omega_w h_s^*X_{s,i} + w_l \sum_i L_i\\
    \text{s.t.}\quad     &\sum_s\sum_{i\in R_s^F} h_s^*X_{s,i}\delta_{s,i}\leq C \label{eq:to_hub_capacity}\\
    &\sum_s\sum_{i\in R_s^T} h_s^*X_{s,i}\delta_{s,i}\leq C \label{eq:from_hub_capacity}\\
    &\sum_s X_{s,i}+L_{i}= \bar{D}_i\\
    & X_{s,i}, \,L_i \geq 0 \label{eq:integer_cons}
\end{aligned}
\end{eqnarray}
while the problem is in general a bilinear programming problem, it becomes a linear programming problem once $h_s^*$ is known as the decisions made by the service planning agency. As a max-min problem, we can convert the inner minimization problem to its dual maximization form as:
\begin{eqnarray}
\begin{aligned}
    \max_{p,\lambda} &\sum_i (\bar{X}_i+p_iZ_i)U_i(t^*,h^*)\lambda_i+\sum_i t_{s,i}g_i+\sum_i\sum_s \kappa_s^*\delta_{s,i} (\bar{X}_i+Z_i)\mu_i\\
    \text{s.t.}\quad & \lambda_i+\mu_i+h_{s,i}^*tb g_i \leq \sum_{s\in\mathcal{R}}(-\omega_se_i-\omega_rc_r)\delta_{s,i}\\
    &\sum_i p_i=T, p_i\in\{0,1\}, \forall\,i\\
    &\lambda_i\leq 0, \mu_i\leq 0,\forall i
    \end{aligned}
\end{eqnarray}
The recourse problem now becomes a bilinear optimization problem. As $p_i$ are binary variables, instead of solving a nonconvex problem, we can further convert this problem into an equivalent MILP by making use of the big-M method and replacing each $p_i\lambda_i$ with $\gamma_i$ as:
\begin{eqnarray}
\begin{aligned}
    \max_{p,\lambda} &\sum_i \sum_s \bar{X}_iU_i(t^*,h^*)\lambda_i+Z_iU_i(t^*,h^*)\gamma_i+\delta_{s,i}t_{s,i}^*g_i+\kappa_s^*\delta_{s,i} (\bar{X}_i+Z_i)\mu_{i}\\
    \text{s.t.}\quad & \lambda_i+\mu_i+t_bh_{s,i}^*\leq \sum_{s\in\mathcal{R}}(-\omega_se_i-\omega_rc_r)\delta_{s,i}\\
    \gamma_i&\leq p_iM\\
    \gamma_i&\leq \lambda_i+(1-p_i)M\\
    &\sum_i p_i=T, p_i\in\{0,1\}, \forall\,i\\
    &\lambda_i\leq 0, \mu_i\leq 0,\forall i
    \end{aligned}
\end{eqnarray}
which is a standard MILP as $\kappa_s^*$ is given and $U_i(t^*,h^*)$ is a constant with known $t^*,h^*$. 

To solve the master problem, the major challenge arises from the bilinear term $y_st_{s,i}$ in the objective function and the bilinear constraint $y_sh_s$ where $y_s$ are integer variables. The bilinear constraints indicate the master problem is a nonconvex integer programming problem. While the objective function is linear in $y,h$, we can instead relax the bilinear term and reformulate the problem as a mixed-integer linear programming problem. As the first step, we introduce the unary expansion of the integer variables as 
\begin{equation}
    y_s=\sum_{k=0}^m 2^k v_s^k, v_s^k\in\{0,1\}, \forall s 
\end{equation}
where we can bound the value of $m$ as $m=\lc log_2(B+1) \rc-1$ with $\lc\cdot\rc$ being the operator for rounding up to the nearest integer. 

As a consequence, we can replace each $y_sh_s$ term with a single variable $z_s$ and have
\begin{equation}
y_sh_s=\sum_{k=0}^m 2^kv_s^kh_s,\forall 
\label{eq:unary}
\end{equation}
and we can further replace $v_s^kh_s$ with $z_s^k$ and deriving the boundary for $z_s^k$ based on the McCormick's envelope:
\begin{eqnarray}
\begin{aligned}
    y_sh_s&=\sum_{k=0}^m 2^kz_s^k \\
    h_s^{min}&\leq z_s^k \leq h_s^{max}\\
    v_s^kh_s^{min}&\leq z_s^k\leq v_s^kh_s^{max}\\
    h_s-h_s^{max}(1-v_s^k)&\leq z_s^k \leq h_s-h_s^{min}(1-v_s^k)
    \label{eq:mccormick}
\end{aligned}
\end{eqnarray}
We note that the McCormick envelope constructed for $z_s^k$ is an exact relaxation due to the binary nature of $v_s^k$, and hence equations~\ref{eq:unary} and~\ref{eq:mccormick} result in an exact relaxation of the binary constraint $y_sh_s$. There is an additional bilinear term associated with $y_st_{s,i}$ in the objective function, where we can replace each $v_s^kt_{s,i}$ with $w_{s,i}^k$ and we have.
\begin{eqnarray}
\begin{aligned}
    y_st_{s,i}&=\sum_{k=0}^m 2^kw_{s,i}^k \\
    t_{s,i}^{min}&\leq w_{s,i}^k \leq t_{s,i}^{max}\\
    v_s^kt_{s,i}^{min}&\leq w_{s,i}^k\leq v_s^kt_{s,i}^{max}\\
    t_{s,i}-t_{s,i}^{max}(1-v_s^k)&\leq w_{s,i}^k \leq t_{s,i}-t_{s,i}^{min}(1-v_s^k)
    \label{eq:mccormick}
\end{aligned}
\end{eqnarray}
With this relaxation, we arrive at the equivalent reformulation of the master problem as a MINLP:
\begin{subequations}
    \begin{align}
    \min_{v,h} \quad & \omega_oc_o\sum_{s\in\mathcal{R}}[T_s^{travel}(\sum_{k=0}^m2^kv_s^k)+\sum_i\delta_{s,i}(\sum_{k=0}^m2^kw_{s,i}^k)]+\eta\\
    &\eta \geq \sum_{s\in\mathcal{R}}\sum_{i\in V}-(\omega_se_i+\omega_rc_r)\delta_{s,i}X_i^l\,,l=1,2,...,L\\
    &t_{s,i}\geq t_b X_i^lh_{s,i}\,,l=1,2,...,L\\
    & X_i^l\leq (\bar{X}_i+p_i^{*l}Z_i)U_i(t,h),\forall\,i, l=1,2,...,L\label{eq:nlcon1}\\
    &X_i^l\leq \sum_s \delta_{s,i}\kappa_s(\bar{X}_i+Z_i), l=1,2,...,L\\
    &\sum_{k=0}^m 2^kz_s^k \geq \kappa_sT_s^{trip}+\sum_i \delta_{s,i}t_{s,i}\\
    &t_{s,i}\leq M \kappa_s\\
    &\sum_{k=0}^m 2^kv_s^k\leq B\kappa_s, \kappa_s\in\{0,1\}\\
    &\sum_s\sum_{k=0}^m 2^kv_s^k \leq B\\
    &v_s^kh_s^{min}\leq z_s^k\leq v_s^kh_s^{max}\\
    &h_s-h_s^{max}(1-v_s^k)\leq z_s^k \leq h_s-h_s^{min}(1-v_s^k)\\
    &v_s^kt_{s,i}^{min}\leq w_{s,i}^k\leq v_s^kt_{s,i}^{max}\\
    &t_{s,i}-t_{s,i}^{max}(1-v_s^k)\leq w_{s,i}^k \leq t_{s,i}-t_{s,i}^{min}(1-v_s^k)\\
    &v_s^k\in\{0,1\},\forall s,k\\
    \end{align}
\end{subequations}
With the given $p^{*L}$, $X^L$ is known explicitly and the set of nonlinear constraints as the function of $T_{s,i}$, hence $y$ and $t$, is described by equation~\ref{eq:nlcon1}. Let $g_i^l(t,h)=p_i^*lZ_iU_i(t,h)$, it is easy to verify that $U_i(t,h)$ is a convex function in $h,t$ for all $i$ and hence $g_i^l(t,h)$ is also convex. 
And we can use CPLEX to solve this problem sequentially. 

\subsection{Solution algorithm}
For the MINLP of the master problem, we use the outer approximation (OA) approach~\cite{duran1986outer} which is known to solve the MINLP to global optimal with convex nonlinear constraint.

For the robust optimization problem, we introduce the following column and generation algorithm~\cite{zeng2013solving}:
\begin{steps}
    \item Initialization; Set $LB=-\inf$, $UB=\inf$; Set T=0, set $\Gamma=\{\}$.
    \item Find an initially feasible $p^0\in\mathcal{P}$, add $p^0$ to $\Gamma$. Set T=1.
    \item Solve master-RCIP($\Gamma$) to global optimum  and obtain $Y^{*},L^{*},\eta^*$; Update $LB=\mathbb{1}^TY^{*}+ h^TL^*+\eta^*$. 
    \item Solve MILP-SubRCIP($Y^{*},L^{*}$) and obtain $p^*$,$z^{*},\mu^{*}$. Update $UB=\mathbbm{1}^TY^{*}+ h^TL^*+ \sum_{k=0}^M 2^k1^Tz^{*k}-HL^{*T}\mu^*$. 
    \item If $UB-LB\leq \delta$, terminate and return $Y^*$ and $L^*$ as the optimal solution of the RCIP problem. Otherwise go to Step 4.
    \item Add $p^*$ to $\Gamma$; set $T=T+1$; go to Step 3.  
\end{steps}
For Step 2, one can simply use the stationary charging probability as a reasonable initial feasible $p^0$ to start the algorithm. The most computationally expensive step of the algorithm is to solve the recourse problem, which we have reformulated from a BLP to a MILP. The algorithm is proved to converge in finite steps and the complete proof can be found in~\cite{zeng2013solving}. Besides the theoretical guarantee, the algorithm is also shown to converge in few iterations in numerous applications, and is found to be much more efficient than an alternative solution method that introduces cutting plane in an iterative manner (e.g., the Kelly's algorithm presented in~\cite{gabrel2014robust}). 

Master-NLP problem
\begin{subequations}
    \begin{align}
    \min_{t,h} \quad &\omega_oc_o\sum_{s\in\mathcal{R}}\sum_i\delta_{s,i}(\sum_{k=0}^m2^kw_{s,i}^k)+\eta\\
    &\eta \geq \sum_{s\in\mathcal{R}}\sum_{i\in V}-(\omega_se_i+\omega_rc_r)\delta_{s,i}X_i^l\,,l=1,2,...,L\\
    &t_{s,i}\geq t_b X_i^{l}h_{s,i}\,,l=1,2,...,L\\
    & X_i^{l}\leq (\bar{X}_i+p_i^{*l}Z_i)U_i(t,h),\forall\,i, l=1,2,...,L\label{eq:nlcon1}\\
    &X_i^l\leq \sum_s \delta_{s,i}\kappa_s^*(\bar{X}_i+Z_i), l=1,2,...,L\\
    &\sum_{k=0}^m 2^kz_s^k \geq \kappa_sT_s^{trip}+\sum_i \delta_{s,i}t_{s,i}\\
    &t_{s,i}\leq M \kappa_s\\
    &h_s-h_s^{max}(1-v_s^{k*})\leq z_s^{k*} \leq h_s-h_s^{min}(1-v_s^{k*})\\
    &v_s^{k*}t_{s,i}^{min}\leq w_{s,i}^k\leq v_s^{k*}t_{s,i}^{max}\\
    &t_{s,i}-t_{s,i}^{max}(1-v_s^{k*})\leq w_{s,i}^k \leq t_{s,i}-t_{s,i}^{min}(1-v_s^{k*})\\
    \end{align}
\end{subequations}

Master-MILP problem
\begin{subequations}
    \begin{align}
    \min_{v,h} \quad & \omega_oc_o\sum_{s\in\mathcal{R}}[T_s^{travel}(\sum_{k=0}^m2^kv_s^k)+\sum_i\delta_{s,i}(\sum_{k=0}^m2^kw_{s,i}^k)]+\eta\\
    &\eta \geq \sum_{s\in\mathcal{R}}\sum_{i\in V}-(\omega_se_i+\omega_rc_r)\delta_{s,i}X_i^l\,,l=1,2,...,L\\
    &t_{s,i}\geq t_b X_i^l\,,l=1,2,...,L\\
    & X_i^l\leq (\bar{X}_i+p_i^{*l}Z_i)((x-x^k)^T\partial U_i(t,h)+U_i(t_0,h_0)),\forall\,i, l=1,2,...,L\label{eq:nlcon1}\\
    &X_i^l\leq \sum_s \delta_{s,i}\kappa_s(\bar{X}_i+Z_i), l=1,2,...,L\\
    &\sum_{k=0}^m 2^kz_s^k \geq \kappa_sT_s^{trip}+\sum_i \delta_{s,i}t_{s,i}\\
    &t_{s,i}\leq M \kappa_s\\
    &\sum_{k=0}^m 2^kv_s^k\leq B\kappa_s, \kappa_s\in\{0,1\}\\
    &\sum_s\sum_{k=0}^m 2^kv_s^k \leq B\\
    &v_s^kh_s^{min}\leq z_s^k\leq v_s^kh_s^{max}\\
    &h_s-h_s^{max}(1-v_s^k)\leq z_s^k \leq h_s-h_s^{min}(1-v_s^k)\\
    &v_s^kt_{s,i}^{min}\leq w_{s,i}^k\leq v_s^kt_{s,i}^{max}\\
    &t_{s,i}-t_{s,i}^{max}(1-v_s^k)\leq w_{s,i}^k \leq t_{s,i}-t_{s,i}^{min}(1-v_s^k)\\
    &v_s^k\in\{0,1\},\forall s,k\\
    \end{align}
\end{subequations}
